Voice Agents: From Auditory Intelligence to Auditory Agency

Voice systems increasingly combine streaming speech, persistent state, reasoning, tool use, and embodied control. Once these functions share a runtime, spoken input can change digital or physical state, and recognition or response quality alone no longer characterizes the system. This article studies the interfaces through which spoken evidence becomes consequential. \emph{Auditory intelligence} denotes the capabilities required to perceive, understand, coordinate, and generate spoken interaction; \emph{auditory agency} denotes the causal path from that interaction to stateful decisions and observable consequences. The \emph{commitment boundary} marks where revisable auditory evidence becomes persistent state, a plan, or an executable request. \emph{Agency closure} then follows an authorized action through observation, verification, recovery or compensation, and communication of the outcome. Evidence from full-duplex interaction, reasoning, memory, tools, embodiment, and human control shows a consistent systems-level mismatch: integration is advancing faster than end-to-end observation of what the integrated system actually does. The resulting design problem is to preserve a trace from spoken evidence to consequence while keeping commitment, execution, and verification attributable.

==> archive/retired_figures/fig3_architecture_families.tex <==
\begin{figure*}[tp]
\centering
\includegraphics[width=\textwidth]{figures/processed/fig3_architecture_image.png}
\caption{Architectural families and the distribution of intelligence in voice agents. The upper panel contrasts cascaded, partially integrated, end-to-end, and native full-duplex or embodied architectures; the lower panel shows how intelligence can reside in a single model, a layered stack, or distributed specialized modules.}
\label{fig:architecture}
\end{figure*}


==> archive/retired_figures/fig6_trustworthy_loop.tex <==
\begin{figure*}[tp]
\centering
\includegraphics[width=0.81\textwidth]{figures/static_generated/fig6_trustworthy_loop.png}
\caption{Trustworthy action loop from spoken intent to verified consequence. Interpretation and grounding precede authorization and execution; observation then supports verification, confirmation, and recovery. Privacy, consent, security, fairness, and accessibility cut across the loop rather than belonging to a single component.}
\label{fig:trust-loop}
\end{figure*}


==> archive/retired_figures/fig8_roadmap.tex <==
\begin{figure*}[tp]
\centering
\includegraphics[width=\textwidth]{figures/processed/fig8_roadmap_image.png}
\caption{Roadmap toward general auditory agency. The figure places today's fragmented capabilities, the current integration frontier, and the longer-term goal of general auditory agency on one trajectory, then grounds that trajectory in the perceive--understand--plan--execute--observe--verify/recover--confirm cycle and its key enablers.}
\label{fig:roadmap}
\end{figure*}


==> archive/retired_tables/table2_architecture_families.tex <==
% Table II: architecture families viewed through ownership of consequential state.
\begin{table*}[tp]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.16}
\caption{Voice-agent architecture families viewed through ownership of state, action, and consequence.}
\label{tab:architecture-families}
\begin{tabularx}{\textwidth}{@{}L{2.1cm} Y Y Y Y@{}}
\toprule
\rowcolor{TableHead}
\textbf{Family} & \textbf{Interaction / state} & \textbf{Decision / action owner} & \textbf{Verification / recovery} & \textbf{Design implication} \\
\midrule
\textbf{Cascade} & text and explicit symbolic state exchanged between modules & dialogue manager; service layer & application or dialogue manager & visible interfaces; accumulated latency and information loss \cite{PAPER_E17F117D3387,PAPER_03CE3B0B842C} \\
\textbf{Speech--language model} & audio, text, or latent speech inside a shared model & shared model; external tools when present & often external or implicit & coherent cross-modal reasoning; less visible decision boundaries \cite{PAPER_190E84406795,PAPER_C5043A3C2B57,PAPER_F09AF490D578} \\
\textbf{Native full duplex} & concurrent acoustic and semantic streams with generation-time control & joint generator; optional downstream controller & generally outside the duplex model & low-latency coordination; interaction and action can become entangled \cite{PAPER_1473A84B8A9D,PAPER_FAE46C323E2F,PAPER_65418243EE76} \\
\textbf{Layered voice agent} & streaming interaction front end plus planner and typed executor & planner plus explicit executor & dedicated verifier or application state & visible commitment and consequence boundaries; stronger interface contracts \cite{PAPER_40A1EF47A5D0,PAPER_B421DE5BB9A8} \\
\textbf{Tool-augmented agent} & speech or text coupled to structured calls and observations & orchestrator or planner plus external service & service response or explicit verifier & rapid capability expansion; authorization and partial failure become central \cite{PAPER_766B59A1727C,PAPER_09240145263B,PAPER_9AD353416653} \\
\textbf{Embodied agent} & speech combined with vision, scene state, and control signals & multimodal policy or planner plus controller & sensors and world state & observable consequence; harder reversibility and human takeover \cite{PAPER_A40BBDA83DC5,PAPER_E9854767F763,EXTERNAL_ELLSA} \\
\bottomrule
\end{tabularx}
\end{table*}


==> archive/retired_tables/table3_agentic_governance_landscape_v26.tex <==
% Table III: consolidated agentic capability + governance landscape.
\begin{table*}[tp]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.06}
\caption{Agentic capabilities and governance constraints organized by the interface they expose. Capability evidence and human-centered constraints are shown together because consequential behavior depends on both what the system can do and the conditions under which that transition is permitted and observable.}
\label{tab:agentic-governance}
\label{tab:reasoning-memory-tools}
\label{tab:trustworthy}
\begin{tabularx}{\textwidth}{@{}L{2.25cm} Y L{2.75cm} Y@{}}
\toprule
\rowcolor{TableHead}
\textbf{Interface} & \textbf{Mechanism or system question} & \textbf{Useful endpoint / horizon} & \textbf{Boundary and representative evidence} \\
\midrule
\rowcolor{TableGroup}
\multicolumn{4}{@{}l}{\textbf{A. State, reasoning, and memory}}\\[-1pt]
\textbf{Explicit state / policy} & symbolic or learned dialogue state with a policy over declared variables & state accuracy; policy return; task success / turn--session & makes decision state inspectable \cite{PAPER_E17F117D3387,PAPER_03CE3B0B842C,PAPER_EC2365EC8FAE} \\
\textbf{Streaming reasoning} & partial transcript, semantic event, or latent speech state triggers deliberation & trigger quality; reasoning quality; latency / turn--session & reasoning can start before a turn is complete, but early hypotheses remain provisional \cite{PAPER_13438B5C64C7,PAPER_CB6C6E4E2062,PAPER_8B3C1EFAB4CB} \\
\textbf{Clarification / replanning} & uncertainty-aware question, revision, or abandonment of a provisional plan & clarification accuracy; revised task outcome / task & distinguishes revising a plan from merely producing another response \cite{PAPER_EC0445D89B24,PAPER_913915B00C96} \\
\textbf{Retrieval memory} & audio- or text-based retrieval into the current interaction & recall; answer accuracy; faithfulness / turn--session & retrieval quality does not establish durable user state \cite{PAPER_76F78E88F459,PAPER_7C61510F1269,PAPER_45B6406FAE17} \\
\textbf{Persistent memory} & preference, episodic, or dual-store memory across sessions & preference use; identity isolation; long-horizon quality / cross-session & persistence creates correction, deletion, provenance, and drift obligations \cite{PAPER_FFAF306C931D,PAPER_07DE94B0DB13,PAPER_4AC64B8C94AB} \\
\addlinespace[2pt]
\rowcolor{TableGroup}
\multicolumn{4}{@{}l}{\textbf{B. Action and consequence}}\\[-1pt]
\textbf{Speech-to-tool mapping} & function selection and structured argument generation from speech & selection and argument accuracy / turn & valid call generation is not execution \cite{PAPER_766B59A1727C} \\
\textbf{Synchronized tool use} & action tokens or structured calls generated on the duplex speech clock & tool accuracy; pass@1; latency / turn--task & timing evidence remains distinct from authorization and side effects \cite{PAPER_09240145263B,PAPER_9AD353416653} \\
\textbf{Typed execution / recovery} & planner dispatches constrained operations with retry or fallback & completion; lifecycle events; fallback behavior / task & execution is observable, but success still requires outcome verification \cite{PAPER_40A1EF47A5D0,PAPER_B421DE5BB9A8} \\
\textbf{Grounded state change} & workflow evaluated against a target environment or database state & achieved-vs.-target state / task & establishes consequence inside the stated environment \cite{PAPER_535B4C25EDC0} \\
\textbf{Embodied action} & dialogue state coupled to navigation, manipulation, or situated control & task outcome; control success; takeover / episode & physical consequence raises reversibility and hand-back requirements \cite{PAPER_A40BBDA83DC5,PAPER_E9854767F763,EXTERNAL_ELLSA} \\
\addlinespace[2pt]
\rowcolor{TableGroup}
\multicolumn{4}{@{}l}{\textbf{C. Human control, security, and deployment}}\\[-1pt]
\textbf{Personalization / memory control} & What user context may persist, and how can it be corrected or removed? & preference use; correction; deletion; drift & useful memory is not equivalent to controllable memory \cite{PAPER_FFAF306C931D,PAPER_07DE94B0DB13,PAPER_4AC64B8C94AB} \\
\textbf{Identity / authorization} & Who is speaking, who is being served, and may this speaker request this action? & verification; unsafe-action rate; correct abstention & recognition is evidence of identity, not permission to act \cite{PAPER_E648C7BE210D,PAPER_BA00BDF2544F,PAPER_40A1EF47A5D0} \\
\textbf{Consent / privacy} & What may be captured, retained, reused, or disclosed? & consent lifecycle; disclosure; reconstruction risk & privacy constraints travel with state, not only with the microphone \cite{PAPER_E5C507BB2EE0,PAPER_49C7AB780EBD,PAPER_1036315221F1} \\
\textbf{Security / availability} & Can adversarial audio, memory, or tool inputs alter or block the loop? & attack success; defence rate; leakage; availability & persistence and action enlarge the attack surface \cite{PAPER_AF925F6B6A7D,PAPER_FFE347059994,PAPER_E62762C38D81} \\
\textbf{Trust / interaction quality} & Do timing, prosody, explanation, and recovery support calibrated reliance? & appropriateness; repeated-interaction reliance & perceived quality cannot substitute for safe or correct action \cite{PAPER_12AD80B5D1F4,PAPER_307D36780825,PAPER_170D457B6045} \\
\textbf{Accessibility / fairness} & Who experiences degraded recognition, synthesis, or interaction quality? & subgroup differences across accent, language, age, and disability & access to the loop is itself a systems constraint \cite{PAPER_A8FB29F113AF,PAPER_F5E043F38380,PAPER_3389FD1BA564} \\
\textbf{High-stakes oversight} & Which decisions require confirmation, escalation, takeover, or professional judgment? & escalation; takeover success; confirmed outcome & workflow fit does not establish domain efficacy \cite{PAPER_6688E5A9A34D,PAPER_D0815A91F238,PAPER_8554E35C4B44} \\
\bottomrule
\end{tabularx}
\end{table*}


==> archive/retired_tables/table3_realtime_duplex.tex <==
% Table III: compact real-time and full-duplex synthesis.
\begin{table*}[tp]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.14}
\caption{Representative design patterns in real-time and full-duplex voice interaction.}
\label{tab:duplex}
\begin{tabularx}{\textwidth}{@{}L{2.45cm} Y Y Y@{}}
\toprule
\rowcolor{TableHead}
\textbf{Representative work} & \textbf{Design pattern} & \textbf{Main evidence} & \textbf{Systems role} \\
\midrule
\rowcolor{TableGroup}
\multicolumn{4}{@{}l}{\textbf{Native and integrated duplex}}\\[-1pt]
Moshi \cite{PAPER_1473A84B8A9D} & parallel codec streams with an internal text stream & continuous listening and speaking; about 160\,ms theoretical latency & native low-delay duplex generation \\
SALM-Duplex; Freeze-Omni \cite{PAPER_FAE46C323E2F,PAPER_65418243EE76} & duplex behavior learned directly or attached to a frozen language model & direct listen/speak control with low-latency dialogue & alternative routes to duplex capability \\
BayLing-Duplex; MinMo \cite{PAPER_9DD954E00CAA,PAPER_F09AF490D578} & autoregressive or unified multimodal voice modeling & native full-duplex dialogue plus broader voice tasks & concurrency inside the shared model \\
\addlinespace[2pt]
\rowcolor{TableGroup}
\multicolumn{4}{@{}l}{\textbf{Modular and consequential interaction}}\\[-1pt]
FlexDuo; DuplexCascade \cite{PAPER_30744A6D4C42,PAPER_9C69E07FE883} & duplex controller layered over an existing back end & pluggable turn coordination & modular alternative to full-model retraining \\
DuplexSLA \cite{PAPER_09240145263B} & synchronized speech, planning, turn labels, and structured calls & 85.56\% tool accuracy at 0.648\,s; 91.33\% at 2.77\,s for a cascade & exposes latency--action trade-offs \\
Full-Duplex-Bench v2/v3 \cite{PAPER_B8CB31F1F27C,PAPER_9AD353416653} & overlap, disfluency, and mocked APIs & duplex interaction plus tool use; $F_1$ 0.876; pass@1 0.600 & connects timing to bounded action traces \\
FD-Bench; IHBench \cite{PAPER_4F97D68B6C26,PAPER_2D9099D449E2} & interruption scenarios and recovery rubrics & interruption handling and post-interruption recovery & separates task success from recovery quality \\
Endpointing and anticipatory control \cite{PAPER_CB8E8D2C7474,PAPER_11D6F89D815C,PAPER_C60EBC02D547,PAPER_82CBE66BE086,PAPER_9DC02CA93758} & semantic completion, barge-in, multi-state turn decisions, and early prediction & turn-state accuracy, barge-in $F_1$, and latency--speculation trade-offs & makes commitment timing explicit \\
\bottomrule
\end{tabularx}
\end{table*}


==> archive/retired_tables/table4_evidence_research_agenda_v26.tex <==
% Table IV: consolidated evaluation endpoints + research agenda.
\begin{table*}[tp]
\centering
\scriptsize
\setlength{\tabcolsep}{3.8pt}
\renewcommand{\arraystretch}{1.07}
\caption{Evidence endpoints and research agenda for auditory agency. Panel A shows how the observable endpoint changes the claim that can be supported; Panel B turns the main unresolved interfaces into experimentally tractable research questions. Values in Panel A retain their original experimental meaning and are not directly comparable.}
\label{tab:evidence-agenda}
\label{tab:results}
\label{tab:roadmap}
\begin{tabularx}{\textwidth}{@{}L{2.15cm} Y L{2.65cm} Y@{}}
\toprule
\rowcolor{TableHead}
\multicolumn{4}{@{}l}{\textbf{A. Representative evidence endpoints}}\\[-1pt]
\textbf{Endpoint} & \textbf{Representative evidence} & \textbf{Reported result} & \textbf{What the evidence establishes} \\
\midrule
\textbf{Signal} & four-state turn classification under the stated test conditions \cite{PAPER_11D6F89D815C} & about 95.75\% mean accuracy & discrimination among pause, backchannel, interruption, and continuation \\
\textbf{Semantic} & streaming intent and slot localization in a closed-set setting \cite{PAPER_C69F6F77FA7A} & about 98.97\% joint accuracy & meaning can be localized before a turn is complete \\
\textbf{Interaction} & barge-in prediction on real IVR audio \cite{PAPER_C60EBC02D547} & macro-$F_1$ 0.826 & when the system should yield; downstream state is not tested \\
\textbf{Task} & synchronized structured actions over 900 cases \cite{PAPER_09240145263B} & 85.56\% tool accuracy at 0.648\,s & low-latency call generation; execution and authorization remain separate \\
\textbf{Consequence} & 278 grounded service tasks with a gold database state \cite{PAPER_535B4C25EDC0} & 31--51\% clean; 26--38\% realistic & achieved simulated state is checked against a target \\
\textbf{Human outcome} & attentive-listening interaction with older adults \cite{PAPER_12AD80B5D1F4} & about 60\% judged appropriate & human-facing appropriateness over short interaction \\
\addlinespace[3pt]
\rowcolor{TableHead}
\multicolumn{4}{@{}l}{\textbf{B. Research directions at unresolved interfaces}}\\[-1pt]
\textbf{Direction} & \textbf{Core systems question} & \textbf{Illustrative experiment} & \textbf{Representative evidence base} \\
\midrule
\textbf{Revisable spoken evidence} & How can partial evidence guide reasoning without making an early interpretation irreversible? & inject natural corrections after provisional planning and trace dependent state revision or cancellation & \cite{PAPER_82CBE66BE086,PAPER_9AD353416653} \\
\textbf{Identity, authority, persistent state} & How should identity, permission, provenance, and time scope travel with decision state? & follow users and memory objects across sessions; test stale state, correction, deletion, and cross-user isolation & \cite{PAPER_4AC64B8C94AB,PAPER_AA174144A864} \\
\textbf{Closing the action loop} & How should planners, executors, and verifiers coordinate under denial, timeout, partial writes, or concurrent change? & evaluate authorization, abstention, post-action state, verification, cancellation, compensation, and escalation in one trace & \cite{PAPER_535B4C25EDC0,PAPER_2D9099D449E2} \\
\textbf{Longitudinal coordination} & How do reliance, correction, accessibility, and hand-back evolve over repeated interaction? & repeated-session studies linking human outcomes to memory, recovery, and user intervention & \cite{PAPER_12AD80B5D1F4,PAPER_3389FD1BA564} \\
\bottomrule
\end{tabularx}
\end{table*}


==> archive/retired_tables/table4_reasoning_memory_tools.tex <==
% Table IV: agentic technologies grouped by visible transition.
\begin{table*}[tp]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.14}
\caption{Representative technologies along the agentic loop, organized by the transition they make observable.}
\label{tab:reasoning-memory-tools}
\begin{tabularx}{\textwidth}{@{}L{2.25cm} Y C{1.8cm} Y Y@{}}
\toprule
\rowcolor{TableHead}
\textbf{Capability} & \textbf{Representative mechanism} & \textbf{Horizon} & \textbf{Typical endpoint} & \textbf{Representative refs.} \\
\midrule
\rowcolor{TableGroup}
\multicolumn{5}{@{}l}{\textbf{State and reasoning}}\\[-1pt]
Explicit state / policy & symbolic or learned dialogue state with a policy over declared variables & turn--session & state accuracy; policy return; task success & \cite{PAPER_E17F117D3387,PAPER_03CE3B0B842C,PAPER_EC2365EC8FAE} \\
Streaming reasoning & partial transcript, semantic event, or latent speech state triggers planning & turn--session & reasoning quality; trigger quality; latency & \cite{PAPER_13438B5C64C7,PAPER_CB6C6E4E2062,PAPER_8B3C1EFAB4CB} \\
Clarification / replanning & uncertainty-aware question, revision, or abandonment of a provisional plan & task & clarification accuracy; task outcome & \cite{PAPER_EC0445D89B24,PAPER_913915B00C96} \\
\addlinespace[2pt]
\rowcolor{TableGroup}
\multicolumn{5}{@{}l}{\textbf{Memory}}\\[-1pt]
Retrieval memory & audio- or text-based retrieval into the current interaction & turn--session & recall; answer accuracy; faithfulness & \cite{PAPER_76F78E88F459,PAPER_7C61510F1269,PAPER_45B6406FAE17} \\
Persistent memory & preference, episodic, or dual-store memory across sessions & cross-session & preference use; identity isolation; long-horizon quality & \cite{PAPER_FFAF306C931D,PAPER_07DE94B0DB13,PAPER_4AC64B8C94AB} \\
\addlinespace[2pt]
\rowcolor{TableGroup}
\multicolumn{5}{@{}l}{\textbf{Action and consequence}}\\[-1pt]
Speech-to-tool mapping & function selection and structured argument generation from speech & turn & selection and argument accuracy & \cite{PAPER_766B59A1727C} \\
Synchronized tool use & action tokens or structured calls generated on the duplex speech clock & turn--task & tool accuracy; pass@1; latency & \cite{PAPER_09240145263B,PAPER_9AD353416653} \\
Typed execution / recovery & planner dispatches constrained operations with retry or fallback & task & completion; execution events; fallback behavior & \cite{PAPER_40A1EF47A5D0,PAPER_B421DE5BB9A8} \\
Grounded state change & workflow evaluated against a target environment or database state & task & pass against specified end state & \cite{PAPER_535B4C25EDC0} \\
Embodied action & dialogue state coupled to navigation, manipulation, or situated control & episode & task outcome; control success; takeover & \cite{PAPER_A40BBDA83DC5,PAPER_E9854767F763,EXTERNAL_ELLSA} \\
\bottomrule
\end{tabularx}
\end{table*}


==> archive/retired_tables/table5_trustworthy.tex <==
% Table V: human-centered constraints on the agency loop.
\begin{table*}[tp]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.15}
\caption{Human-centered constraints expressed at the interfaces of an action-capable voice-agent loop.}
\label{tab:trustworthy}
\begin{tabularx}{\textwidth}{@{}L{2.35cm} Y Y Y@{}}
\toprule
\rowcolor{TableHead}
\textbf{Constraint} & \textbf{System question} & \textbf{Useful endpoint} & \textbf{Representative refs.} \\
\midrule
\rowcolor{TableGroup}
\multicolumn{4}{@{}l}{\textbf{State, identity, and authority}}\\[-1pt]
Personalization / memory & What user context may persist, and how can it be corrected or removed? & preference use; correction; deletion; long-horizon drift & \cite{PAPER_FFAF306C931D,PAPER_07DE94B0DB13,PAPER_4AC64B8C94AB} \\
Identity / authorization & Who is speaking, who is being served, and is this speaker authorized for this action? & verification; unsafe-action rate; correct abstention & \cite{PAPER_E648C7BE210D,PAPER_BA00BDF2544F,PAPER_40A1EF47A5D0} \\
Consent / privacy & What may be captured, retained, reused, or disclosed? & consent lifecycle; disclosure; reconstruction risk & \cite{PAPER_E5C507BB2EE0,PAPER_49C7AB780EBD,PAPER_1036315221F1} \\
\addlinespace[2pt]
\rowcolor{TableGroup}
\multicolumn{4}{@{}l}{\textbf{Interaction and robustness}}\\[-1pt]
Security / availability & Can adversarial audio, memory, or tool inputs alter or block the loop? & attack success; defence rate; leakage; availability & \cite{PAPER_AF925F6B6A7D,PAPER_FFE347059994,PAPER_E62762C38D81} \\
Trust / interaction quality & Do timing, prosody, explanation, and recovery support calibrated reliance? & appropriateness; reliance over repeated interaction & \cite{PAPER_12AD80B5D1F4,PAPER_307D36780825,PAPER_170D457B6045} \\
Accessibility / fairness & Who experiences degraded recognition, synthesis, or interaction quality? & subgroup differences across accent, language, age, and disability & \cite{PAPER_A8FB29F113AF,PAPER_F5E043F38380,PAPER_3389FD1BA564} \\
\addlinespace[2pt]
\rowcolor{TableGroup}
\multicolumn{4}{@{}l}{\textbf{Deployment oversight}}\\[-1pt]
High-stakes use & Which decisions require confirmation, escalation, takeover, or professional judgment? & escalation; takeover success; confirmed outcome & \cite{PAPER_6688E5A9A34D,PAPER_D0815A91F238,PAPER_8554E35C4B44} \\
\bottomrule
\end{tabularx}
\end{table*}


==> archive/retired_tables/table6_quantitative.tex <==
% Table VI: representative evidence endpoints across the evaluation discussion.
\begin{table*}[tp]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.16}
\caption{Representative evidence endpoints used in the evaluation discussion. Values retain their original experimental meaning and are not directly comparable.}
\label{tab:results}
\begin{tabularx}{\textwidth}{@{}L{1.75cm} Y L{2.55cm} Y@{}}
\toprule
\rowcolor{TableHead}
\textbf{Endpoint} & \textbf{Representative evidence} & \textbf{Reported result} & \textbf{What the evidence establishes} \\
\midrule
\textbf{Signal} & four-state turn classification under the stated test conditions \cite{PAPER_11D6F89D815C} & about 95.75\% mean accuracy & discrimination among pause, backchannel, interruption, and continuation \\
\textbf{Semantic} & streaming intent and slot localization in a closed-set setting \cite{PAPER_C69F6F77FA7A} & about 98.97\% joint accuracy & meaning can be localized before a turn is complete \\
\textbf{Interaction} & barge-in prediction on real IVR audio \cite{PAPER_C60EBC02D547} & macro-$F_1$ 0.826 & when the system should yield; downstream state is not tested \\
\textbf{Task} & synchronized structured actions over 900 cases \cite{PAPER_09240145263B} & 85.56\% tool accuracy at 0.648\,s & low-latency call generation; execution and authorization remain separate \\
\textbf{Consequence} & 278 grounded service tasks with a gold database state \cite{PAPER_535B4C25EDC0} & 31--51\% clean; 26--38\% realistic & achieved simulated state is checked against a target \\
\textbf{Human outcome} & attentive-listening interaction with older adults \cite{PAPER_12AD80B5D1F4} & about 60\% judged appropriate & human-facing appropriateness over short interaction \\
\bottomrule
\end{tabularx}
\end{table*}


==> archive/retired_tables/table7_roadmap.tex <==
% Table VII: compact research agenda.
\begin{table*}[tp]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.16}
\caption{Research agenda derived from the interfaces that govern auditory agency.}
\label{tab:roadmap}
\begin{tabularx}{\textwidth}{@{}L{2.85cm} Y Y@{}}
\toprule
\rowcolor{TableHead}
\textbf{Direction} & \textbf{Core systems question} & \textbf{Illustrative experiment} \\
\midrule
\textbf{Revisable spoken evidence} & How can partial evidence guide reasoning without making an early interpretation irreversible? & inject natural corrections after provisional planning; trace which dependent states and prepared actions are revised or cancelled \cite{PAPER_82CBE66BE086,PAPER_9AD353416653} \\
\textbf{Identity, authority, and persistent state} & How should identity, permission, provenance, and time scope travel with the state used for a decision? & follow users and memory objects across sessions; test stale state, correction, deletion, and cross-user isolation \cite{PAPER_4AC64B8C94AB,PAPER_AA174144A864} \\
\textbf{Closing the action loop} & How should planners, executors, and verifiers coordinate when services deny, time out, partially write, or change concurrently? & evaluate authorization, abstention, post-action state, verification, cancellation, compensation, and escalation in one trace \cite{PAPER_535B4C25EDC0,PAPER_2D9099D449E2} \\
\textbf{Longitudinal human--agent coordination} & How do reliance, correction, accessibility, and hand-back evolve when the same user interacts with the same agent over time? & repeated-session studies linking human outcomes to changes in agent state, memory, recovery behavior, and user intervention \cite{PAPER_12AD80B5D1F4,PAPER_3389FD1BA564} \\
\bottomrule
\end{tabularx}
\end{table*}


==> figures/fig4_interaction_loop.tex <==
\begin{figure*}[tp]
\centering
\includegraphics[width=0.81\textwidth]{figures/static_generated/fig4_interaction_loop.png}
\caption{Full-duplex spoken interaction as a revisable loop. Perception and source attribution feed incremental understanding and turn prediction; listening and speaking are then coordinated across a commitment boundary, while interruption and correction can trigger semantic repair and replanning. The stages are analytical functions rather than a fixed implementation pipeline.}
\label{fig:interaction-loop}
\end{figure*}


==> figures/fig5_agent_loop.tex <==
\begin{figure*}[tp]
\centering
\includegraphics[width=\textwidth]{figures/processed/fig5_action_closure_image.png}
\caption{Closed-loop interaction-to-consequence pipeline and an evidence ladder for action closure. The upper panel traces the path from interaction and commitment to action closure and user-confirmed consequence. The lower panel shows why execution, observation, verification, and recovery require different forms of evidence.}
\label{fig:agent-loop}
\end{figure*}

